The Photometric LSST Astronomical Time-series Classification Challenge (PLAsTiCC): Data set

The Photometric LSST Astronomical Time Series Classification Challenge (PLAsTiCC) is an open data challenge to classify simulated astronomical time-series data in preparation for observations from the Large Synoptic Survey Telescope (LSST), which will achieve first light in 2019 and commence its 10-year main survey in 2022. LSST will revolutionize our understanding of the changing sky, discovering and measuring millions of time-varying objects. In this challenge, we pose the question: how well can we classify objects in the sky that vary in brightness from simulated LSST time-series data, with all its challenges of non-representativity? In this note we explain the need for a data challenge to help classify such astronomical sources and describe the PLAsTiCC data set and Kaggle data challenge, noting that while the references are provided for context, they are not needed to participate in the challenge.

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar
#
# Alex Drlica-Wagner: https://github.com/LSSTDESC/start_paper/issues/new?body=@kadrlica

# Primary file names - avoid cookiecutter variables, to enable `make
# upgrade` to cleanly over-write this Makefile...
main ?= main
#default=$(shell cat .metadata.json | grep 'default_format' | cut -d'"' -f4)
outname ?= $(notdir $(shell pwd))

#ifeq ($(default), {{ cookiecutter.default_format }})
style ?= lsstdescnote
#else
# style=${default}
#endif

# 'note' shall be an alias for 'lsstdescnote'
ifeq ($(style),note)
style = lsstdescnote
endif
# mkauthlist doesn't recognize lsstdescnote as a style, so tell it to do something generic
ifeq ($(style),lsstdescnote)
mastyle = tex
else
mastyle = $(style)
endif

DESCTEX := desc-tex
DESCTEXORIGIN := git@github.com:LSSTDESC/desc-tex.git
LSSTTEX := lsst-texmf
LSSTTEXORIGIN := git@github.com:lsst/lsst-texmf.git

localpip ?= F
PIPOPTS = --upgrade-strategy only-if-needed
ifeq ($(localpip),T)
MKAUTHBIN := bin/mkauthlist
MKAUTH := PYTHONPATH=$$(ls -d lib/python*/site-packages 2>/dev/null | head -n1):$$PYTHONPATH $(MKAUTHBIN)
PIPOPTS += --install-option="--prefix=$(PWD)"
GETMKAUTH := [ -e $(MKAUTHBIN) ] || pip install $(PIPOPTS) mkauthlist
else
MKAUTHBIN :=
MKAUTH := mkauthlist 
GETMKAUTH := pip list 2>/dev/null | grep -q mkauthlist || pip install $(PIPOPTS) mkauthlist
endif

# LATEX environment variables
export TEXINPUTS:=./$(DESCTEX)/styles/:./tables/:
export BSTINPUTS:=./$(DESCTEX)/bst/:
export BIBINPUTS:=./$(DESCTEX)/bib/:./$(LSSTTEX)/texmf/bibtex/bib/:

# LaTeX journal class switcher flags
# apj=\def\flag{apj}
# apjl=\def
# mnras=\def\flag{mnras}

# Submission flags (these need some thought)
# arxiv=\def\flag{emulateapj}
# submit=${aastex}
# draft=\def\linenums{\linenumbers}

# Files to copy when making tarball
tardir := tmp
figdir ?= ./figures
figures ?= $(figdir)/*.{png,jpg,pdf}
tabdir ?= ./tables
tables ?= $(tabdir)/*.tex
styles ?= ./$(DESCTEX)/styles/*.{sty,cls}
bibs ?= ./$(DESCTEX)/bib/*.bst
source = $(main).{tex,bbl,bib} $(DESCTEX)/bib/lsstdesc.bib $(DESCTEX)/ack/*.tex authors.tex contributions.tex $(LSSTTEX)/texmf/bibtex/bib/lsst.bib $(LSSTTEX)/texmf/bibtex/bib/lsst-dm.bib

tarfiles = $(figures) $(tables) $(styles) $(bibs) $(source)

# prefix for difference files
DIFPRE ?= diff_
# git repo branch to compare changes against
BASEBRANCH ?= master
# git repo branch we are compiling
THISBRANCH := $(shell git branch --no-color 2> /dev/null | sed -e '/^[^*]/d' -e 's/* \(.*\)/ \1/' | tr -d ' ')
# temp file for the version to compare against
DRAFT = $(main).$(BASEBRANCH)
# base for difference files to generate
DIFF = $(DIFPRE)$(THISBRANCH)--$(BASEBRANCH)


maketargets := all authlist clean copy diff help $(main) update tar templates tidy touch
.PHONY: $(maketargets)

styleopts := aastex61 apj apjl emulateapj lsstdescnote mnras note prd prl tex 
help:
	@echo "Usage: make [style=lsstdescnote] [localpip=F] <target(s)>\n Possible targets: $(maketargets) <style> $(DESCTEX) $(LSSTTEX)\n  all: equivalent to 'make $(main) copy'\n  authlist: use mkauthlist to generate latex author/affiliation listing\n  clean: remove latex temporary files AND compiled outputs\n  copy: copy $(main).pdf to $(outname).pdf\n  diff: if we're in a git repo, use latexdiff to compare the current $(main).tex vs the $(BASEBRANCH) branch, and attempt to compile to $(DIFF).pdf\n  help: what you're looking at\n  $(main): compile $(main).tex\n  update: update desc-tex, mkauthlist, and templates repo\n  tar: tar up latex source files to $(outname).tar.gz\n  templates: download latest templates to templates/\n  tidy: delete latex temporary files\n  touch: touch $(main).tex to force a recompile\n  <style>: equivalent to 'make style=<style> $(main) copy tar' (see style option)\n  $(DESCTEX): download $(DESCTEX), which provides the DESC header logo and latex helper files (done automatically on first latex compilation)\n  $(LSSTTEX): download $(LSSTTEX), providing (among other things) LSST project bib files (not done automatically)\n Options for style: $(styleopts) (Anything else results in generic latex)\n Options for localpip: T or F. Set to T to install mkauthlist in this directory rather than systemwide"


# Interpret `make` with no target as `make tex` (a latex Note).
# At present, if the default_format is anything other than
# [apj|apjl|mnras|prd|prl|emulateapj], a latex Note is made.
# In future, we could think of using `make` to eg run the ipynb
# notebook and make PDF from the output, but this has not been
# implemented yet.
$(main): export flag = \def\flag{${style}}
envflag = \\def\\flag{${style}}
all: $(main) copy

copy:
	cp ${main}.pdf ${outname}.pdf

touch:
	touch ${main}.tex

# if we are in a git repo, add as a submodule; otherwise clone
$(DESCTEX):
	if [ -d .git ]; then git submodule add $(DESCTEXORIGIN); else git clone $(DESCTEXORIGIN); fi
$(LSSTTEX):
	if [ -d .git ]; then git submodule add $(LSSTTEXORIGIN); else git clone $(LSSTTEXORIGIN); fi

#http://journals.aas.org/authors/aastex/linux.html
#change the compiler call to allow a "." file
# {% raw %}
$(main) : $(DESCTEX) authlist
	STYLEFLAG=$(envflag) latexmk $(main)
#	latexmk -g -pdf  \
	-pdflatex='openout_any=a pdflatex %O -interaction=nonstopmode "${flag}\input{%S}"'  \
	${main}
# {% endraw %}

diff: $(DIFF).pdf
$(DIFF).pdf: $(DIFF).tex
	STYLEFLAG=$(envflag) latexmk $<
$(DIFF).tex: $(DRAFT).tex $(main).tex
	latexdiff --exclude-textcmd="multicolumn" $^ > $@
# this ensures that the version to latexdiff against is always updated
.PHONY: $(DRAFT).tex
$(DRAFT).tex:
	if git show $(BASEBRANCH):$(main).tex > $@; then true; else echo "\n\n'make diff' is intended to be used inside a git repository\n"; false; fi



tar : $(main)
	mkdir -p ${tardir}
	cp ${tarfiles} ${tardir} | true
	cp ${outname}.pdf ${tardir}/${outname}.pdf
	cd ${tardir} && tar -czf ../${outname}.tar.gz . && cd ..
	rm -rf ${tardir}

authlist: authors.tex
authors.tex : authors.csv
	$(GETMKAUTH)
	$(MKAUTH) -j ${mastyle} -f -c "LSST Dark Energy Science Collaboration" \
		--cntrb contributions.tex authors.csv authors.tex
#	pip install --upgrade mkauthlist


# http://stackoverflow.com/q/8028314/
.PHONY: $(styleopts)
$(styleopts): export style = $(@)
$(styleopts): export flag = \def\flag{$(@)}
$(styleopts):
	$(MAKE) -e $(main)
	$(MAKE) -e copy
	$(MAKE) -e tar
# NB. the 'tex' target doesn't actually do anything in docswitch - make
# with no target compiles PDF out of main.tex using lsstdescnote.cls
# (which is to say, by default we assume you are writing an LSST
# DESC Note in latex format).

tidy:
	rm -f *.log *.aux *.out *.dvi *.synctex.gz *.fdb_latexmk *.fls
	rm -f *.bbl *.blg *Notes.bib ${main}.pdf

clean: tidy
	rm -f ${outname}.pdf ${outname}.tar.gz

# Update the tex styles etc:

baseurl=https://raw.githubusercontent.com/LSSTDESC/start_paper/deploy

# UPDATES=\
# texmf/bib/apj.bst \
# texmf/bib/mnras.bst \
# texmf/styles/aas_macros.sty \
# texmf/styles/aastex.cls \
# texmf/styles/aastex61.cls \
# texmf/styles/aps_macros.sty \
# texmf/styles/docswitch.sty \
# texmf/styles/emulateapj.cls \
# texmf/styles/mnras.cls \
# texmf/styles/lsstdescnote.cls \
# texmf/styles/lsstdesc_macros.sty \
# texmf/logos/desc-logo-small.png \
# texmf/logos/desc-logo.png \
# texmf/logos/header.png \
# lsstdesc.bib \
# .travis.yml \
# figures/example.png

# .PHONY: $(UPDATES)
# $(UPDATES):
# 	curl -s -S -o $(@) ${baseurl}/$(@)
# 	@echo " "

update: templates
	@echo Updating desc-tex
	cd $(DESCTEX) && git pull
	@echo
	@echo Updating mkauthlist
	pip install --upgrade $(PIPOPTS) mkauthlist
#@echo "\nOver-writing LaTeX style files with the latest versions: \n"
#@mkdir -p .logos figures texmf/styles texmf/bib
#$(MAKE) $(UPDATES)

# Get fresh copies of the templates etc, for reference:
# It is a bad idea to make these phony targets

TEMPLATES:=\
authors.csv \
main.ipynb \
main.md \
main.rst \
main.tex \
main.bib \
Makefile
#.metadata.json \
#.travis.yml 
#figures/example.png
# #acknowledgments.tex \

ALLTEMPLATES := $(TEMPLATES) header.png

# .PHONY: $(TEMPLATES)
# $(TEMPLATES):
# 	curl -s -S -o templates/$(@) ${baseurl}/$(@)
# 	@echo " "

gettemplates := $(foreach t,$(TEMPLATES),curl -s -S -o templates/$(t) ${baseurl}/$(t); )

# NB: fetching header.png will fail as long as desc-tex is private
templates:
	@echo "\nDownloading the latest versions of the template files, for reference: \n"
	@mkdir -p templates
	$(gettemplates)
	curl -f -s -S -o templates/header.png https://raw.githubusercontent.com/LSSTDESC/desc-tex/master/logos/header.png || true
	@echo
	@echo templates/ listing:
	@ls -a templates/*
	@for f in $(ALLTEMPLATES); do diff -q $$f templates/$$f; true; done
#$(MAKE) $(TEMPLATES)
#	$(MAKE) new

# Get a template copy of the latest Makefile, for reference:
# new:
# 	@echo "\nDownloading the latest version of the Makefile, for reference: \n"
# 	@mkdir -p templates
# 	curl -s -S -o templates/Makefile ${baseurl}/Makefile
# 	@echo " "

# Over-write this Makefile with the latest version:
# Why would we include this when a safe option already exists?
# upgrade:
# 	@echo "\nDownloading the latest version of the Makefile: \n"
# 	curl -s -S -o Makefile ${baseurl}/Makefile
# 	@echo "\nUpgrading version of mkauthlist: \n"
# 	pip install mkauthlist --upgrade --no-deps
# 	@echo "\nNow get the latest styles and templates with\n\n    make update\n    make templates\n"


==> authors.tex <==
% Author list
\vspace{4\baselineskip}

%\noindent{\href{http://www.plasticcblog.wordpress.com}{\LARGE\bf Contributing Authors}}

%\clearpage
%\vspace{5\baselineskip}

% List of institutions:
\def\adler{Adler Planetarium, \ldots}
\def\arizona{U of Arizona, \ldots}
\def\caltech{California Institute of Technology, \ldots}
\def\centrallancashire{University of Central Lancashire, UK, \ldots}
\def\cfa{Harvard-Smithsonian Center for Astrophysics, \ldots}
\def\cmu{Carnegie Mellon University, \ldots}
\def\columbia{Columbia, \ldots}
\def\cuny{CUNY, \ldots}
\def\ctio{Cerro Tololo Inter-American Observatory, La Serena, Chile}
\def\dearborn{University of Michigan-Dearborn, \ldots}
\def\delaware{University of Delaware, \ldots}
\def\drexel{Drexel University, \ldots}
\def\ennu{NU, \ldots}
\def\floridagulf{Florida Gulf Coast University, \ldots}
\def\goddard{NASA Goddard Space Flight Center, \ldots}
\def\harvard{Department of Physics, Harvard University, \ldots}
\def\ifa{Institute for Astronomy, Honolulu, HI \ldots}
\def\ipac{IPAC, \ldots}
\def\jpl{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA 91109, USA, \ldots}
\def\lcogt{LCOGT, University of California, Santa Barbara, CA \ldots}
\def\lsst{LSST, \ldots}
\def\msu{Michigan State, \ldots}
\def\nso{National Solar Observatory, \ldots}
\def\noao{NOAO, \ldots}
\def\nyu{New York University, NY, \ldots}
\def\osu{Ohio State University, \ldots}
\def\oswego{State University of New York at Oswego, \dots}
\def\oxford{University of Oxford, UK, \ldots}
\def\penn{University of Pennsylvania, \ldots}
\def\princeton{Department of Astrophysical Sciences, Princeton University, Princeton, NJ 08544, USA}
\def\rutgers{Rutgers, \ldots}
\def\scsu{Southern Connecticut State University, \ldots}
\def\seti{SETI Institute, \ldots}
\def\slac{SLAC National Accelerator Laboratory, 2575 Sand Hill Road, MS29, Menlo Park, CA 94025, USA}
\def\somewhere{Some Institute, Somewhere, \ldots}
\def\stanford{Physics Department, Stanford University, Stanford, CA, 94305, USA}
\def\stsci{STScI, \ldots}
\def\texastech{Texas Tech University, \ldots}
\def\ucd{University of California, Davis, \ldots}
\def\ucl{UCL, \ldots}
\def\unab{UNAB, Chile, \ldots}
\def\unt{University of North Texas, \ldots}
\def\usno{USNO, \ldots}
\def\utaustin{University of Texas at Austin, \ldots}
\def\uw{University of Washington, \ldots}
\def\westernwash{Western Washington University, \ldots}
\def\vanderbilt{Vanderbilt University, \ldots}
\def\yale{Yale University, \ldots}
\def\toronto{Department of Astronomy and Astrophysics \& Dunlap Institute, University of Toronto}
\def\stockholm{Oscar Klein Center, Stockholm University}

% List of authors:
\author{The PLAsTiCC team:}
\affiliation{Corresponding author: \href{mailto:hlozek@dunlap.utoronto.ca}{hlozek@dunlap.utoronto.ca}}
\author{Tarek Allam Jr.}
\affiliation{Mullard Space Science Laboratory, Department of Space and Climate Physics, University College London, Holmbury Hill Rd, Dorking RH5 6NT, UK}
\author{Anita Bahmanyar}
\affiliation{Department of Astronomy and Astrophysics \& Dunlap Institute for Astronomy and Astrophysics,  University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{Rahul Biswas}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}
\author{Mi Dai}
\affiliation{Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854 USA}
\author{Llu\'is Galbany}
\affiliation{University of Pittsburgh, 300 Allen Hall, 3941 O'Hara St, Pittsburgh, PA 15260}
\author{Ren\'ee Hlo\v{z}ek}
\affiliation{Department of Astronomy and Astrophysics \& Dunlap Institute for Astronomy and Astrophysics,  University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{Emille E.~O.~Ishida}
\affiliation{Universit\'e Clermont Auvergne, CNRS/IN2P3, LPC, F-63000 Clermont-Ferrand, France}
\author{Saurabh~W.~Jha}
\affiliation{Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854 USA}
\author{David~O.~Jones}\affiliation{Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 92064, USA}
\author{Richard Kessler}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago,
IL 60637, USA}
\author{Michelle Lochner}
\affiliation{African Institute for Mathematical Sciences, 6 Melrose Road, Muizenberg, 7945, South Africa}
\affiliation{South African Radio Astronomy Observatory, The Park, Park Road, Pinelands, Cape Town 7405, South Africa}
\author{Ashish A. Mahabal}
\affiliation{Division of Physics, Mathematics, and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{Center for Data Driven Discovery, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Alex~I.~Malz}
\affiliation{Center for Cosmology and Particle Physics, New York University, 726 Broadway, New York, NY 10004, USA}
\affiliation{Department of Physics, New York University, 726 Broadway, New York, NY 10004, USA}
\author{Kaisey~S.~Mandel}
\affiliation{Institute of Astronomy and Kavli Institute for Cosmology, Madingley Road, Cambridge, CB3 0HA, UK}
\affiliation{Statistical Laboratory, DPMMS, University of Cambridge, Wilberforce Road, Cambridge, CB3 0WB, UK}
\author{Juan Rafael Mart\'inez-Galarza}
\affiliation{Harvard-Smithsonian Center for Astrophysics, 60 Garden Street,Mail Stop 66 Cambridge, MA 02138}
\author{Jason~D.~McEwen}
\affiliation{Mullard Space Science Laboratory, Department of Space and Climate Physics, University College London, Holmbury Hill Rd, Dorking RH5 6NT, UK}
\author{Daniel Muthukrishna}
\affiliation{Institute of Astronomy and Kavli Institute for Cosmology, Madingley Road, Cambridge, CB3 0HA, UK}
\author{Gautham Narayan}
\affiliation{Space Telescope Science Institute, 3700 San Martin Dr, Baltimore, MD 21218, USA}
\author{Hiranya Peiris}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}
\affiliation{Department of Physics and Astronomy, University College London, Gower Street, London, WC1E 6BT, UK }
\author{Christina M. Peters}
\affiliation{Department of Astronomy and Astrophysics \& Dunlap Institute for Astronomy and Astrophysics,  University of Toronto, 50 St. George St., Toronto, ON M5S 3H4, Canada}
\author{Kara Ponder}
\affiliation{Berkeley Center for Cosmological Physics, Campbell Hall 341, University of California Berkeley, Berkeley, CA 94720, USA}
\author{Christian~N.~Setzer}
\affiliation{The Oskar Klein Centre for Cosmoparticle Physics, Stockholm University, AlbaNova, Stockholm, SE-106 91, Sweden}
\collaboration{(LSST Dark Energy Science Collaboration and the LSST Transients and Variable Stars Science Collaboration)}
\vspace{8\baselineskip}



==> key.tex <==
The DESC acknowledges ongoing support from the Institut National de Physique Nucl\'eaire et de Physique des Particules in France; the Science \& Technology Facilities Council in the United Kingdom; and the Department of Energy, the National Science Foundation, and the LSST Corporation in the United States.  DESC uses resources of the IN2P3 Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la Recherche Scientifique; the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported by the Office of Science of the U.S.\ Department of Energy under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BIS National E-infrastructure capital grants; and the UK particle physics grid, supported by the GridPP Collaboration.  This work was performed in part under DOE Contract DE-AC02-76SF00515.


==> latexmkrc <==
# Choose which style to pass to docswitch
# NB: Default value here is always used by Overleaf
$theflag = $ENV{'STYLEFLAG'} || '\def\flag{lsstdescnote}';

# Set environment variables to search for tex inputs
# http://tex.stackexchange.com/a/50847/121099
$ENV{'TEXINPUTS'}='./desc-tex/:./tables/:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./desc-tex/bib/:' . $ENV{'BSTINPUTS'};

# Set control tools
$go_mode = 1;
$pdf_mode = 1;
# You can change the \flag value here...
$pdflatex = 'openout_any=a pdflatex %O -interaction=nonstopmode "' . $theflag . '\input{%S}"'


==> standard_short.tex <==
DESC acknowledges ongoing support from the IN2P3 (France), the STFC (United Kingdom), and the DOE, NSF, and LSST Corporation (United States).  DESC uses resources of the IN2P3 Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la Recherche Scientifique; the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BIS National E-infrastructure capital grants; and the UK particle physics grid, supported by the GridPP Collaboration.  This work was performed in part under DOE Contract DE-AC02-76SF00515.

